Cross-Domain Empirical Risk Minimization for Unbiased Long-tailed Classification

We address the overlooked unbiasedness in existing long-tailed classification methods: we find that their overall improvement is mostly attributed to the biased preference of tail over head, as the test distribution is assumed to be balanced; however, when the test is as imbalanced as the long-tailed training data -- let the test respect Zipf's law of nature -- the tail bias is no longer beneficial overall because it hurts the head majorities. In this paper, we propose Cross-Domain Empirical Risk Minimization (xERM) for training an unbiased model to achieve strong performances on both test distributions, which empirically demonstrates that xERM fundamentally improves the classification by learning better feature representation rather than the head vs. tail game. Based on causality, we further theoretically explain why xERM achieves unbiasedness: the bias caused by the domain selection is removed by adjusting the empirical risks on the imbalanced domain and the balanced but unseen domain. Codes are available at https://github.com/BeierZhu/xERM.

==> images/KD.tex <==
\begin{figure}[t]
    \centering
     \includegraphics[width=0.38\textwidth]{images/compareKD.pdf}
    \caption{Comparisons with a varying constant weight $w$ on CIFAR100-LT-IB-50 dataset.}
    \label{fig:figKD}
\end{figure}

==> images/compareKD.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{images/CompareKD.pdf}
\caption{Comparison of the top-1 accuracy when varying weight $w$ of the knowledge distillation method on CIFAR100-LT, IB50 dataset.}
\label{fig:figKD}
\end{wrapfigure}

==> images/gamma.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.38\textwidth]{images/Gamma.pdf}
    \caption{Comparisons with a varying gamma $\gamma$ in Eq.~\eqref{eq:wfcf} on CIFAR100-LT-IB-50 dataset.}
    \label{fig:gamma}
\end{figure}

==> tables/ShiftedCifarImageNet.tex <==
\begin{minipage}{\textwidth}
\begin{minipage}[t]{0.45\textwidth}
\makeatletter\def\@captype{table}
\centering
\caption{Top-1 accuracy over all classes on imbalanced CIFAR100-LT test set.}
\label{tab:LTtestCIFAR100}
\scalebox{0.9}{
\begin{tabular}{l|cccc}
\shline
Imbalance ratio                 & 100 & 50   & 10   & 5                       \\ \hline
% CE                            & 67.0 & 65.1 & 57.3 & 52.8  & 40.5                 \\
BBN                             & 58.0 & 56.3 & 52.5 & 49.3                  \\
LADE                            & 59.5 & 57.6 & 53.3 & 51.5                   \\
PC                              & 60.0 & 59.2 & 55.3 & 52.9                   \\
cRT                             & 60.8 & 59.5 & 55.0 & 52.0                    \\
TDE                             & 60.8 & 60.0 & 55.7 & 52.9                  \\ \hline
XE                              & \tbf{66.4} & 63.9 & 56.3 & 51.9                  \\ \hline
\textbf{xERM}$_{\!P\!C}$ & 63.3 & 61.5 & 57.0 & 54.6  \\
\textbf{xERM}$_{\!T\!D\!E}$    & \tbf{66.4} & \tbf{64.8} & \tbf{59.3} & \tbf{55.5}     \\ \shline
\end{tabular}}
\end{minipage}
\hspace{1em}
\begin{minipage}[t]{0.45\textwidth}
\makeatletter\def\@captype{table}
\centering
\caption{Top-1 accuracy over all classes on imbalanced ImageNet-LT test set.}
\label{tab:LTtestImageNet}
\scalebox{0.9}{
\begin{tabular}{l|cccc}
\shline
Imbalanced ratio                  & 50            & 25            & 10            & 5                                             \\ \hline
$\tau$-Norm                       & 59.6          & 58.2          & 56.2          & 54.6         \\
LWS                               & 60.6          & 59.2          & 57.0          & 55.0           \\
PC                                & 58.2          & 56.8          & 54.5          & 52.7           \\
LADE                              & 61.8          & 60.6          & 58.6          & 56.8           \\ 
TDE                               & 63.0          & 61.6          & 59.5          & 57.6           \\ \hline
XE                                & \textbf{67.7} & 65.2          & 61.4          & 58.0           \\ \hline
\textbf{xERM}$_{\!P\!C}$ & 66.8          & 65.3          & 62.5          & 60.1           \\
\textbf{xERM}$_{\!T\!D\!E}$    & \textbf{67.7} & \textbf{66.0} & \textbf{63.5} & \textbf{60.9}   \\ \shline
\end{tabular}}
\end{minipage}
\end{minipage}

==> tables/longtailTestCifar.tex <==
\begin{table}[t]
\centering
\caption{Top-1 accuracy over all classes on long-tailed, uniform and reversed long-tailed CIFAR100-LT-IB-50 test set.}
% \vspace{1em}
\vspace{2mm}
\begin{tabular}{l|llll|l|llll}
\shline
Dataset         & \multicolumn{4}{c|}{Long-tailed}              & Uni.                & \multicolumn{4}{c}{Reversed Long-tailed}                                                                                   \\ \hline
Imbalance ratio  & \multicolumn{1}{c}{50} & \multicolumn{1}{c}{25} & \multicolumn{1}{c}{10} & \multicolumn{1}{c|}{5} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{25} & \multicolumn{1}{c}{50} \\ \hline
XE                                      & 66.0  & 63.5 & 59.0  & 55.4  &  45.1  &  35.1  & 31.1  & 26.8  & 24.4      \\ 
PC$^\mathrm{cfb}$                       & 61.5  & 60.3 & 57.4  & 55.6  &  49.7  &  44.2  & 41.8  & 39.7  & 38.5      \\ 
PC$^\mathrm{cfi}$                       & 56.8  & 56.1 & 54.0  & 53.0  &  49.6  &  47.1  & 45.7  & 44.7  & 43.8        \\\hline
\tbf{FCF-ERM}                           & 62.6  & 60.9 & 58.2  & 56.6  &  51.7  &  46.9 &  44.8  & 42.9  & 42.1 \\ \shline
\end{tabular}
\label{tab:beyond}
\end{table}
